Accurate Coresets for Latent Variable Models and Regularized Regression

Accurate coresets are a weighted subset of the original dataset, ensuring a model trained on the accurate coreset maintains the same level of accuracy as a model trained on the full dataset. Primarily, these coresets have been studied for a limited range of machine learning models. In this paper, we introduce a unified framework for constructing accurate coresets. Using this framework, we present accurate coreset construction algorithms for general problems, including a wide range of latent variable model problems and $\ell_p$-regularized $\ell_p$-regression. For latent variable models, our coreset size is $O\left(\mathrm{poly}(k)\right)$, where $k$ is the number of latent variables. For $\ell_p$-regularized $\ell_p$-regression, our algorithm captures the reduction of model complexity due to regularization, resulting in a coreset whose size is always smaller than $d^{p}$ for a regularization parameter $\lambda > 0$. Here, $d$ is the dimension of the input points. This inherently improves the size of the accurate coreset for ridge regression. We substantiate our theoretical findings with extensive experimental evaluations on real datasets.

==> section/caratheodory.tex <==
\section{Carathéodory's Theorem for Low Rank Matrix}

\begin{theorem}[Carathéodory's Theorem for Low Rank Matrix]
A derived form of Carathéodory's theorem can be stated as follows: if a point $x \in \mathbb{R}^d$ lies inside the convex hull of a set $P \subset \mathbb{R}^d$, where $|P| = n$ and the rows of $P$ span a $k$-dimensional subspace of $\mathbb{R}^d$, then there is a subset of at most $k+1$ points from $P$ that contains $x$ in its convex hull.
\end{theorem}

\begin{proof}
Let $P$ be a set of points in $\mathbb{R}^d$, with rank $k<d$ and let $x$ be a point in the convex hull of $P$. We can express $x$ as a convex combination of points in $P$:
\[x = \alpha_1p_1 + \alpha_2p_2 + \cdots + \alpha_np_n\]
where $\alpha_1 + \cdots + \alpha_n = 1$, $\alpha_i \geq 0$ for all $i$, and $p_1, \ldots, p_n \in P$.

Now, let's consider the rank of the space. By the rank-nullity theorem, we know that:
\[\text{rank}(A) + \text{nullity}(A) = d\]
where $A$ is the matrix formed by the vectors $p_1, \ldots, p_n$ as columns.

If $n > k+1$, then:
\[\text{nullity}(A) = d - \text{rank}(A) > 0\]
This means there exists a non-zero vector $\beta = (\beta_1, \ldots, \beta_n)$ in the null space of $A$. In other words:
\[\sum_{i=1}^n \beta_i p_i = 0\]

We can use this to show that the points are linearly dependent. Let's construct a linear combination of the points that equals zero:
\[\sum_{i=1}^n \beta_i (p_i - p_1) = 0\]
This is equivalent to:
\[\sum_{i=2}^n \beta_i (p_i - p_1) = 0\]
which is the same form as in the convex hull proof.

Now, we can follow the same steps as in the convex hull proof to reduce the number of points in the convex combination. Define:
\[J = \{i \in \{1,2,\ldots,n\} : \beta_i > 0\}\]
Since $\sum_{i=1}^n \beta_i = 0$ (because $\sum_{i=1}^n \beta_i p_i = 0$ and the $p_i$ are linearly independent), $J$ is not empty. Define:
\[a = \max_{i \in J} \frac{\alpha_i}{\beta_i}\]
Then we can write:
\[x = \sum_{i=1}^n (\alpha_i - a\beta_i)p_i\]
This is a convex combination with at least one zero coefficient. Therefore, we can express $x$ as a convex combination of $n-1$ points.

We can repeat this process until $\text{nullity}(A) = d - \text{rank}(A) = 0$.
In $\mathbb{R}^d$, $\text{nullity}(A) = d - \text{rank}(A) = 0$ holds true if and only if the number of rows of $A$ is less than or equal to $k+1$, where $k$ is the dimension of the space in which the matrix operates.

This proves that if we have more than $k+1$ points in a space of rank $k$, they are linearly dependent, and any point in their convex hull can be expressed as a convex combination of at most $k+1$ of these points.
\end{proof}
